Overcoming High Frequency Limitations of Current-Mode Control Using a Control Conditioning Approach -- Part II: Implementation and Hardware

This article is the second part of a paper series about interference in extremum (i.e., peak or valley) current-mode control, which applies to both fixed and variable switching frequency power converters. Specifically, this part presents three control conditioning methods that mitigate the adverse effect of interference. These methods are new ways to use: (i) slope compensation; (ii) low-pass filtering; and (iii) the phenomenon of comparator-overdrive-delay, for control conditioning. The stability criterion, closed-loop dynamics, and transient performance are derived with mathematical rigor for each method. The design tradeoffs are illustrated, discussed, and compared. The effectiveness of all three methods are demonstrated and validated in hardware using a power converter operating at multi-MHz switching frequencies.

==> 3_modeling.tex <==
%\section{Control Conditioning Approach} \label{sec:modeling}

